Deep-Unrolling Multidimensional Harmonic Retrieval Algorithms on Neuromorphic Hardware

This paper explores the potential of conversion-based neuromorphic algorithms for highly accurate and energy-efficient single-snapshot multidimensional harmonic retrieval (MHR). By casting the MHR problem as a sparse recovery problem, we devise the currently proposed, deep-unrolling-based Structured Learned Iterative Shrinkage and Thresholding (S-LISTA) algorithm to solve it efficiently using complex-valued convolutional neural networks with complex-valued activations, which are trained using a supervised regression objective. Afterward, a novel method for converting the complex-valued convolutional layers and activations into spiking neural networks (SNNs) is developed. At the heart of this method lies the recently proposed Few Spikes (FS) conversion, which is extended by modifying the neuron model's parameters and internal dynamics to account for the inherent coupling between real and imaginary parts in complex-valued computations. Finally, the converted SNNs are mapped onto the SpiNNaker2 neuromorphic board, and a comparison in terms of estimation accuracy and power efficiency between the original CNNs deployed on an NVIDIA Jetson Xavier and the SNNs is being conducted. The measurement results show that the converted SNNs achieve almost five-fold power efficiency at moderate performance loss compared to the original CNNs.

==> definitions.tex <==
%% Font ------------------------------------------------------------
\DeclareMathAlphabet{\mathbit}{OML}{cmr}{bx}{it}
\DeclareMathAlphabet{\mathss}{T1}{cmss}{m}{sl}	% RV
\DeclareMathAlphabet{\mathbss}{T1}{cmss}{bx}{sl}% RV bold
%\newcommand{\rv}[1]{{\mathss #1}}
\newcommand{\brv}[1]{{\mathbss #1}}


\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\Var}{Var}


%% Math commands ---------------------------------------------------
\renewcommand{\jmath}{\mathrm{j}}
\renewcommand{\Re}{\mathrm{Re}\xspace}
\renewcommand{\Im}{\mathrm{Im}\xspace}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\tra}{\mathrm{T}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\unit}{\mathrm{unit}}
\newcommand{\mat}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\st}{\mathrm{s.\,t.}}


%% Sets -------------------------------------------------------------
\newcommand{\D}{\mathcal{D}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Omegaset}{\mathbb{\Omega}}
\newcommand{\Hset}{\mathcal{H}}
\newcommand{\Hnull}{\mathcal{H}_0}
\newcommand{\Halt}{\mathcal{H}_1}

%% Standard Matrices and vectors ------------------------------------
\newcommand{\id}{\mathbf{I}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}

%% Constants --------------------------------------------------------
\newcommand{\Ns}{N_\mathrm{S}}
\newcommand{\Nb}{N_\mathrm{B}}
\newcommand{\Nbar}{\bar{N}}

%% Scalars ----------------------------------------------------------
\newcommand{\Perr}{P_\mathrm{e}}


%% Vectors and matrices (latin) -------------------------------------
\newcommand{\A}{\mathbit{A}}
\newcommand{\V}{\mathbit{V}}
\newcommand{\Cv}{\mathbit{C}}

\newcommand{\Eop}{\mathbit{\hat{E}}}
\newcommand{\aop}{\mathbit{\hat{a}}}
\newcommand{\as}{\mathbit{\hat{a}}_\mathrm{S}}
\newcommand{\ai}{\mathbit{\hat{a}}_\mathrm{I}}
\newcommand{\ab}{\mathbit{\hat{a}}_\mathrm{B}}
\newcommand{\ar}{\mathbit{\hat{a}}_\mathrm{R}}
\newcommand{\nop}{\mathbit{\hat{n}}}
\newcommand{\pop}{\mathbit{\hat{p}}}
\newcommand{\qop}{\mathbit{\hat{q}}}
\newcommand{\xop}{\mathbit{\hat{x}}}
\newcommand{\kv}{\mathbit{k}}
\newcommand{\rv}{\mathbit{r}}
\newcommand{\x}{\mathbit{x}}
\newcommand{\xbar}{\bar{\x}}
\newcommand{\y}{\mathbit{y}}



%% Random variables -------------------------------------------------


%% Vectors and matrices (greek) -------------------------------------
\newcommand{\Pivec}{\ensuremath{\boldsymbol{\Pi}}\xspace}
\newcommand{\Omegavec}{\ensuremath{\boldsymbol{\Omega}}\xspace}
\newcommand{\omegavec}{\ensuremath{\boldsymbol{\omega}}\xspace}
\newcommand{\rhovec}{\ensuremath{\boldsymbol{\rho}}\xspace}
\newcommand{\muvec}{\ensuremath{\boldsymbol{\mu}}\xspace}
\newcommand{\xivec}{\ensuremath{\boldsymbol{\xi}}\xspace}



==> sections/extended_abstract/conclusions.tex <==
We casted the MHR problem as a sparse recovery problem, and solved it using the recently proposed S-LISTA algorithm. We developed a novel method for converting the complex-valued convolutional layers and activations in S-LISTA into SNNs based on the recent FS conversion.
At last, the converted SNNs were mapped onto the SpiNNaker2 neuromorphic board, and a comparison in terms of support recovery error and power efficiency between the original CNNs, deployed on embedded GPU, and the SNNs was conducted. The measurement results show that the converted SNNs can achieve much better power efficiency at moderate performance loss compared to the original CNNs.  

==> sections/extended_abstract/intro.tex <==
% Main points
% \begin{enumerate}
%     \item Importance of MHR in wireless (radar, ISAC)
%     \item Why accurate, single-snapshot algorithms? (low num samples in high mobility scenarios)
%     \item Why compressed sensing? (good reconstruction quality with few measurements, performance guarantees, inherently single-snapshoi) Why deep unrolling? (addresses problems associated with CS, i.e. high computational complexity, high number of iterations, dependence on a pre-specified grid, exponential increase in dictionary size with dimensions, etc., is data-driven, thus enables adaptivity due to model mismatches )
%     \item Why neuromorphic? (energy efficient, bio-inspired, i.e. potentially better performance than ANNs)
% \end{enumerate}
% Problems with current SoA/SNNs
% \begin{enumerate}
%     \item Energy and power efficiency central themes in both wireless and computing (decadal plan, etc.) 
%     \item No competitive learning algorithms for SNNs due to reasons in Alex MA - need for conversion
%     \item Current conversion methods are mostly limited to image classification tasks and networks with ReLU activation function - need for FS conversion
%     \item Currently no methods support complex-valued representations or general regression objectives - need for our work
% \end{enumerate}
% Contributions
% \begin{enumerate}
%     \item Extend S-LISTA approach with multiple neural operators
%     \item Propose conversion framework for complex valued CNNs and activations by extending the FS framework
%     \item Map said conversion on real-neuromorphic hardware
%     \item Performance and power efficiency comparison between SNNs on S2 and ANNs on Jetson
% \end{enumerate}
% Multidimensional Harmonic Retrieval (MHR) is an ubuquitous problem in signal processing, finding applications in radar, and wireless joint communications and sensing among others. Due to the growing bandwidths and high mobility scenarios, it is desirable to develop MHR methods which require one or very few samples. In this sense, compressed sensing (CS) has been an attractive solution due to its good reconstruction qualities and performance guarantees. On the other hand, such approaches incur high computational complexity with increased resolution and relatively slow convergence, which impact both latency and energy efficiency. To address the former, the paradigm of deep unrolling was proposed, a data-driven, deep-learning (DL) approach, where the iterations of CS are unfolded and paramterized by deep neural networks (DNNs), exhibiting good flexibility and performance with lower computational burden. These approaches often deployed on Graphics Processing Units (GPUs) suffer from high energy consumption. To mitigate this, neuromorphic computing platforms such as the SpiNNaker2 were developed, which are very much suited for Spiking Neural Network (SNN) computations, an inherently energy-efficient approach inspired by the sparsity in brain computations. On the other hand, due to the absence of competitive learning algorithms for SNNs, DNN-to-SNN conversion needs to be performed. Although effective conversion methods exist, these are mostly limited to real-valued image classification tasks and DNNs with ReLU activation function, and do not support inherent complex-valued regression tasks inherent to signal processing applications. 
% In this paper, we explore the potentials of deep-unrolling based algorithms deployed on neuromorphic hardware. To this end, we employ the recent S-LISTA DNN to solve MHR tasks, which we then convert to an SNN. We develop a novel extension to the recently proposed few spikes FS neuron model, which is able to approximate complex activations over a bounded domain. Using this neuron model, we finally convert the trained DNNs to SNNs. Lastly, these are evaluated in terms of support recovery error and energy efficiency when deployed on GPUs and real neuromorphic hardware. We experimentally show that SNN-based methods on neuromorphic hardware exhibit much higher power efficiency at a moderate loss of performance. 
Multidimensional Harmonic Retrieval (MHR) is crucial in signal processing for radar, wireless communications, and sensing. In dynamic scenarios with limited samples, compressed sensing (CS) offers good performance but comes with high computational complexity \cite{dimitri2010tensor, liu2022integrated}. Deep unrolling \cite{monga2021algorithm}, a deep-learning approach, parameterizes CS iterations with neural networks, enhancing flexibility and performance at lower computational cost. However, deep unrolling methods on GPUs consume significant energy. Neuromorphic platforms like SpiNNaker2 \cite{gonzalez_spinnaker2_2024} offer energy-efficient Spiking Neural Network (SNN) computations, but lack competitive learning algorithms, requiring conversion from Deep Neural Networks (DNNs). Existing conversion methods are limited to real-valued classification tasks with ReLU activation functions \cite{rueckauer_conversion_2017, sengupta_going_2019, cao_spiking_2015}, unsuited for complex-valued signal processing. In this paper, we explore deep unrolling-based algorithms on neuromorphic hardware. Using the S-LISTA \cite{fu2021structured} DNN, we solve MHR tasks and convert it to an SNN using a novel extension to the few spikes FS \cite{stockl_optimized_2021} neuron model, supporting arbitrary complex activations on a bounded domain. We evaluate these methods in terms of support recovery error and energy efficiency on GPUs and neuromorphic hardware, showing around $\SI{768}{\milli\watt}$ better power efficiency with SNN-based methods on neuromorphic hardware.

==> sections/extended_abstract/proposed_method.tex <==
% Main points
% \begin{enumerate}
%     \item Training strategy for DNNs (Preprocessing, Learning objective) - done
%     \item FS conversion extension to complex case for activations and layers - done
%     \item General algorithm (Post training quantization, Spike generation, i.e. FS with identity function, population and projection creation and weight assignment) - done
% \end{enumerate}
In order to leverage the enhanced paralellism and energy-efficiency of neuromorphic platforms, we convert the trained models to SNNs. For this, the complex-valued and activations need to be converted into neuron models, also called spike coding strategies. We now present our proposed extension of the FS coding scheme \cite{stockl_optimized_2021}, which sends serialized binary codes over a fixed number of time steps $2K$ to approximate an arbitrary activation $f(s) : \mathcal{B} \mapsto \mathbb{C}$ over a bounded domain $\mathcal{B} \subset \mathbb{C}$. The internal dynamics of the neuron model are governed by:
\begin{align}
    v_{\Re}(t + 1) &= v_{\Re}(t) - h_{\Re}(t)z(t), \\    
    z(t) &= \Theta(v_{\Re}(t) - T_{\Re}(t)),
\end{align}
for $t = 1, 3, \dots, 2K - 1$ and
\begin{align}
    v_{\Im}(t + 1) &= v_{\Im}(t) - h_{\Im}(t)z_{\Im}(t), \\    
    z(t) &= \Theta(v_{\Im}(t) - T_{\Im}(t)),
\end{align}
for $t = 2, 4, \dots, 2K$ respectively. The approximation is then computed as
\begin{align}
    \hat{f}(z) = \sum_{t=1}^{K} (d_{\Re}(t) z_{\Re}(t) + \mathrm{j} \cdot d_{\Im}(t) z_{\Im}(t))  .
\end{align}
In this formulation, $d_{\Re}, h_{\Re}, T_{\Re}, d_{\Im}, h_{\Im}, T_{\Im} \in \mathbb{R}^K$ represent parameters associated with the real and imaginary parts of the FS neurons, and $\Theta(\cdot)$ is the Heaviside function. Furthermore $v_{\Re, \Im}(t)$ and $z(t)$ represent the membrane potentials and the generated spikes.
In order to get a good approximation over $\mathcal{B}$, $B$ points are sampled and  following optimization problem is solved analogously to \cite{stockl_optimized_2021}
\begin{align}\label{eq:}
    \min_{\substack{d_{\Re}, h_{\Re}, T_{\Re},\\ 
    d_{\Im}, h_{\Im}, T_{\Im} \in \mathbb{R}^K}} 
    \sum_{i=1}^{B} \lvert f(s_{i}) - \hat{f}(s_{i}) \rvert^{2}.  
\end{align}

The complete conversion, depicted in Figure \ref{fig:snn_slista} goes as follows: First, we perform quantization of the CNN weights, then create the neuron populations and projections by extracting the connection information between these populations. Afterwards, the soft-threshold operators in \eqref{eq:st} are approximated for each layer using the FS neuron model optimized for the specific threshold $\alpha_t$ with \eqref{eq:}. At inference time, the spikes are generated by first re-scaling each sample as $\bm{y} = \beta \frac{\bm{y}}{\lVert\bm{y}\rVert_2}$, with $\beta > 0$ and then generating the spikes according to the FS neuron model applied to $f(s) = s$.  
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/SNN ResLISTA.png}
    \caption{Flowgraph of converted SNN.}
    \label{fig:snn_slista}
\end{figure}

==> sections/extended_abstract/results.tex <==
% Main points 
% \begin{enumerate}
%     \item Function approximation plots (dependence on K)
%     \item Conversion error (CNN and local, metric is support recovery error)
%     \item Power measurements (Mean Inference Time, GPU and S2)
% \end{enumerate}
We first evaluate the proposed neuron model in terms of function approximation capabilities. Figure \ref{fig:fs_training} shows the real and imaginary parts of the true and approximated function, as well as the error for different timesteps $K$. We observe that the proposed method empirically approximates the functions quite well. Furthremore, the number of timesteps required to get a good approximation is below $30$, which makes the method promising regarding delay and energy efficiency.

We now present the task performance and power efficiency results for the converted SNNs on the Spinnaker2 neuromorphic board for $P=1$ sources. Due to the very strict memory limitations of the 1-chip evaluation board, we were only able to map S-LISTA models for $M=1$-D HR problems with a maximum of $T = 5$ layers.

Table \ref{tab:performance} shows the support recovery error, i.e. 
\begin{align}
 \text{SRE} =
  \frac{1}{D}\sum_{d=1}^{D} \frac{\left|\{l \neq l'\ | l \in \text{supp}(\bm{\hat{b}}_d), l' \in \text{supp}(\bm{b}_d)\}\right|}{
\text{supp}(\bm{b})
}
\end{align}
of the two approaches. While the CNN is able to perfectly recover all sources, the converted SNN shows a drop in performance of at most $0.27$. This is due to the imperfect approximations by the FS neurons as well as due to quantization effects. These can be partly mitigated by employing a bigger $\beta$ and sampling $\mathcal{B}$ more finely.

Table \ref{tab:power_eff} shows the power measurements for inference only conducted on the NVIDIA Jetson Xavier NX \cite{nvidia2024} and the experimental SpiNNaker2 \cite{gonzalez_spinnaker2_2024} boards. To get good estimates, we isolated inference events from all other processes by incorporating sufficient sleep times. The reported values were recorded using provided APIs and stem from the CPU/GPU \cite{nvidia2024} for the and from the V05/V08 \cite{gonzalez_spinnaker2_2024} power rails respectively. We observe that the SpiNNaker2 board consumes almost $\SI{768}{\milli\watt}$ less power than the embedded GPU, and since the inference delays were quite similar, we can also infer a better energy efficiency at a moderate performance loss.
\begin{figure}
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/soft_threshold.png}
    \end{subfigure}
    % \hspace*{-0.1\textwidth}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/sigmoid.png}
    \end{subfigure}
    % \hspace*{-0.1\columnwidth}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/cardioid.png}
    \end{subfigure}
    \caption{FS neuron approximating eq. \eqref{eq:st} ($\alpha = 1$), complex-valued sigmoid and cardioid functions for values of $K \in [10, 30]$. Blue denotes the true function, orange the approximation.}
    \label{fig:fs_training}
\end{figure}
\begin{table}
\centering
\begin{center}
\begin{tabular}{|c|c|c|} 
\hline
& CNN & SNN\\
\hline
\hline
No scaling & 0.01 & 0.23 \\
\hline
Scale $\beta=5$ & 0.00 & 0.27 \\
\hline
Scale $\beta=30$ & 0.00 & 0.17 \\
\hline
\end{tabular}
\end{center}
\caption{SRE for $P=1$ sources averaged over $\sigma^2$ $\in [10, 30]\, \text{dB}$.}
\label{tab:performance}
\end{table}
\begin{table}
\centering
\begin{center}
\begin{tabular}{|c|c|c|} 
\hline
Board & Mean Power (\SI{}{\milli\watt}) & Std. (\SI{}{\milli\watt})\\
\hline
\hline
Jetson Xavier NX (CNN) & 1022.33 & 35.95 \\
\hline
SpiNNaker2 (SNN) & 260.35  & 0.16 \\  
\hline
\end{tabular}
\end{center}
\caption{Power consumption of the two approaches.}
\label{tab:power_eff}
\end{table}

==> sections/extended_abstract/sys_model.tex <==
% Main points
% Main points
% \begin{enumerate}
%     \item MHR problem stated mathematically - done
%     \item Sparse recovery with l0-l1 norms - done
%     \item FISTA Loop, difference between FISTA and LISTA (Toeplitz structure enables data-drivenness and efficient impl. by neural operators) - done
%     \item SNNs general + S2 description
% \end{enumerate}
% We consider following abstract form of the MHR problem.
Let $\bm{\xi}_{p} = [\xi_{1p}, \xi_{2p}, \dots, \xi_{Mp}]^{\top} \in [-\frac{1}{2}, \frac{1}{2}]^{M}$ be the parameters associated to a source $p=1,\dots, P$. Let $N_{1}, N_{2}, \dots N_{M}$ represent the number of sensors used to capture each dimension and $N = \prod_{m=1}^{M} N_{m}$. 
% The noisy measurement model of the single-snapshot MHR (SS-MHR) can be given as:
% \begin{align}\label{eq:sys_vec}
%     \bm{y} = \sum_{p=1}^{P} b_{p} \bm{a}_{1}(\xi_{1p}) \otimes \dots \otimes \bm{a}_{M}(\xi_{Mp}) + \bm{z}
% \end{align}
% where $\bm{y}\in\mathbb{C}^{N}, b_{p} \in\mathbb{C}$, and $\bm{z} \sim \mathcal{N}(\bm{0}, \sigma^{2}\bm{\mathrm{I}})\in\mathbb{C}^{N}$ a zero-mean Gaussian noise vector. 
With $\bm{a}_{m}(\xi_{mp}) \in \mathbb{C}^{N_{m}}$ and
\begin{align}
    \left(\bm{a}_{m}(\xi_{mp})\right)_{k} = \mathrm{e}^{-\mathrm{j}2\pi \xi_{mp} k}, \quad k = 0, \dots N_{m} - 1.
\end{align}
and the matrices
\begin{align}
    \bm{A}_{m}(\bm{\xi}) = [\bm{a}_{m}(\xi_{m1}), \dots, \bm{a}_{m}(\xi_{mP})] \in \mathbb{C}^{N_{m}\times P},
\end{align} the measurement model is given by \cite{dimitri2010tensor}
\begin{align}\label{eq:sys_kr}
    \bm{y} &= \left(\bm{A}_{1}(\bm{\xi}) \ast \cdots \ast \bm{A}_{M}(\bm{\xi})\right)\bm{b} + \bm{z} \\
    &= \bm{A}(\bm{\xi})\bm{b} + \bm{z},
\end{align}
where $\ast$ denotes the Khatri-Rao (KR) product, $\bm{b} = [b_{1}, \dots, b_{P}]^{\top}\in\mathbb{C}^{P}$ and $\bm{z} \sim \mathcal{N}(\bm{0}, \sigma^{2}\bm{\mathrm{I}})\in\mathbb{C}^{N}$. The goal of SS-MHR is to estimate the harmonics $\{\bm{\xi}_{p}\}_{p=1}^{P}$ given the measurement $\bm{y}$. 
Since the number of sources is in general unknown, in the sparse recovery paradigm, $L\gg N$ harmonics $\bm{\xi}_{l}$ are chosen, then an oversampled dictionary $\bm{A}(\bm{\xi}) \in \mathbb{C}^{N\times L}$ is constructed Equation \eqref{eq:sys_kr}. Subsequently, the parameters are estimated from the nonzero indices of the sparse solution found by solving 
\begin{align}\label{eq:p1}
    \min_{\bm{b}\in\mathbb{C}^{L}} \left\lVert \bm{y} - \bm{A}(\bm{\xi})\bm{b} \right\rVert_{2}^{2} - \lambda\lVert \bm{b} \rVert_{1},
\end{align}
which theoretically yields near-optimal estimates \cite{beck2009fista}.
A popular approach to solving this is given by the Fast Iterative and Shrinkage Algorithm (FISTA) \cite{beck2009fista}, which at each iteration $t=1,\dots,T$ constructs a solution as
\begin{align}
    \bm{b}_t = \mathcal{S}_{\frac{\lambda}{C}}\left(\bm{W}^{1}_{t} \bm{y} + \bm{W}^{2}_{t} \bm{b}_{t-1}\right)
\end{align}
where $\bm{W}^{1}_{t}=\bm{A}^{H}(\bm{\xi}), \, \bm{W}^{2}_{t} = \bm{I} - \frac{1}{C}\bm{A}^{H}(\bm{\xi})\bm{A}(\bm{\xi}), C=\lambda_{\text{max}}(\bm{A}^{H}(\bm{\xi})\bm{A}(\bm{\xi}))$ and
\begin{align}\label{eq:st}
    \mathcal{S}_{\alpha}(\bm{x}) = \text{sign}(\bm{u}) \max(\lvert\bm{u}\rvert - \alpha, \bm{0})
\end{align}
is the elementwise soft-thresholding operator with $\alpha > 0$.
This approach drastically improves the convergence of traditional ISTA, but needs a high number of iterations to reach a sparse solution $\hat{\bm{b}}$.

In order to address this issue, the Structured Learned ISTA (S-LISTA) was proposed in \cite{fu2021structured}, depicted in Figure \ref{fig:slista} which unfolds the iterations of FISTA and replaces the matrices $\bm{W}^{1}_{t},\bm{W}^{2}_{t}$ with CNNs and considers the threshold $\alpha_t = \frac{\lambda}{C}$ as a trainiable parameter. This is motivated by the fact that, the matrix $\bm{W}^{2}_{t}$ is block-Toeplitz, thus the matrix-vector multiplication is implemented by an $M$-D convolution with separable kernels, which is a fast and efficient operation on modern GPUs. Given a training dataset $\mathcal{D} = \{(\bm{y}_{d}, \bm{b}_{d})\}_{d}^{D}$, the resulting networks are trained using following supervised objective:
\begin{align}
    \mathcal{L}(\bm{b}_d , \hat{\bm{b}}_d) = \frac{1}{D}\sum_{d=1}^{D} \dfrac{\lVert\bm{b}_d -  \hat{\bm{b}}_d \rVert_{2}^{2}}{\lVert\bm{b}_d \rVert_2^{2}}
\end{align}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/ResLISTA.png}
    \caption{Schematic representation of S-LISTA architecture.}
    \label{fig:slista}
\end{figure}

==> sections/poster/intro_motivation.tex <==
% \vspace{8mm}
 % \textcolor{red}{TODO: \begin{enumerate}
 %     \item MHR ubiquitous problem, accurate, computationally and energy efficient solutions needed
 %     \item Example: Joint range and DoA estimation Monostatic MIMO-OFDM radar (picture)
 %     \item CS and DL accurate but not energy efficient -> neuromorphic promising
 %     \item SNNs energy efficient only ReLu activations, classification task, no complex valued processing
 %     \item Contributions: 1. bridge the gap, energy-efficient and accurate complex valued signal processing,
 %     2. extension of neuron model \cite{stockl_optimized_2021} to trainable, adaptive, complex-valued computations 
 %     3. performance and power measurements on real hardware, no estimation
 % \end{enumerate}}
 \begin{itemize}
     \item Multidimensional Harmonic Retrieval (MHR) indispensable for future radar sensing and communication systems!
        \vspace{1cm}
        \begin{figure}
         \centering
         \includegraphics[width=0.5\linewidth]{figures/monostatic_isac.pdf}
         \caption*{Joint Range and Angle Estimation in MIMO-OFDM Radar}
         % \label{fig:example}
        \end{figure}
     % \item \textbf{Example}: Joint Range and Angle Estimation in MIMO-OFDM Radar.
     \item Few-snapshot, accurate, computationally- and energy-efficient methods!
     \begin{itemize}
         % \item Subspace/Tensor methods very accurate, but slow and use lots of snapshots!
         % \item Compressed Sensing accurate, single-snapshot possible, but slow!
         \item Existing algorithms fulfill at most two of the criteria! 
         \item Deep Unrolling accurate, faster, single-snapshot possible, but training data needed and potentially energy-inefficient!
     \end{itemize}
     % \vspace{1cm}
     % \begin{table}
     % \hspace{-2.4cm}
     % % [width=0.5\linewidth]
     %     % \centering
     %     \resizebox{.8\textwidth}{!}{
     %     \begin{tabular}{|p{15cm}|p{15cm}|p{15cm}|}
     %     % {|p{8cm}|p{10cm}|p{10cm}|}
     %     % {|c|c|c|}
     %          \hline
     %          \hspace{1.5em} Method & \hspace{1.5em} \textcolor{green}{Pros} & \hspace{1.5em}\textcolor{red}{Cons} \\
     %          \hline
     %          \begin{itemize}
     %              \item[] Subspace/Tensor 
     %          \end{itemize}
     %           & \begin{itemize}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Accurate to very accurate}
     %          \end{itemize}  &
     %          \begin{itemize}
     %              \item[\textcolor{red}-] \textcolor{red}{Usually slow}
     %              \item[\textcolor{red}-] \textcolor{red}{Lots of snapshots}
     %              \item[\textcolor{red}-] \textcolor{red}{Energy-inefficient}
     %          \end{itemize}\\
     %          \hline
     %          \begin{itemize}
     %              \item[ ] Sparse Recovery 
     %          \end{itemize}
     %           & \begin{itemize}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Accurate}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Single-shapshot}
     %          \end{itemize} & \begin{itemize}
     %              \item[\textcolor{red}-] \textcolor{red}{Usually slow}
     %              \item[\textcolor{red}-] \textcolor{red}{Energy-inefficient}
     %          \end{itemize} \\
     %          \hline
     %          \begin{itemize}
     %              \item[] Deep Unrolling
     %          \end{itemize} \vspace{-1cm}& \begin{itemize}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Accurate}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Single-shapshot}
     %              \item[\textcolor{green}{+}] \textcolor{green}{Usually Fast}
     %          \end{itemize}\vspace{-1cm} & 
     %          \begin{itemize}
     %              \item[\textcolor{red}-] \textcolor{red}{Labeled data}
     %              \item[\textcolor{red}-] \textcolor{red}{Energy-inefficient}
     %          \end{itemize}\vspace{-1cm}\\
     %          \hline
     %     \end{tabular}
     %     }
     %     % \caption*{Caption}
     %     % \label{tab:my_label}
     % \end{table}
     % \vspace{1cm}
    \item \textbf{Solution:} Spiking Neural Networks (SNNs) on Neuromorphic Chips
    \begin{itemize}
        \item Massively parallel, energy-efficient computing, trained as DNNs
        \item Limitations: Simple, real-valued tasks with ReLU activations
    \end{itemize}
    \item \textbf{Our Contributions:}
    \begin{enumerate}
        \item Deep Unrolling-based method for MHR on SNNs.
        \item Novel neuron model for approximating complex-valued activations.
        \item Real-world power measurements on SpiNNaker2 board.
    \end{enumerate}
 \end{itemize}
 

==> sections/poster/method.tex <==
\begin{itemize}
    \item Novel few-spikes (FS) \cite{stockl_optimized_2021} neuron for activation $f(s) : \mathcal{B} \mapsto \mathbb{C}$ over a bounded domain $\mathcal{B} \subset \mathbb{C}$.
    \begin{align}\label{eq:fs_cmplx}
    v_{\Re}(t + 1) &= v_{\Re}(t) - h_{\Re}(t)z_{\Re}(t), \,\, &z_{\Re}(t) = \Theta(v_{\Re}(t) - T_{\Re}(t)), \\
    v_{\Im}(t + 1) &= v_{\Im}(t) - h_{\Im}(t)z_{\Im}(t), \,\, &z_{\Im}(t) = \Theta(v_{\Im}(t) - T_{\Im}(t)),
\end{align}
for $t = 0, \dots, K - 1$ with voltages $v_{\Re}(0) = \Re\{s\}, v_{\Im}(0) = \Im\{s\}$. 
\item Activation approximated as
% \begin{align}
%     v_{\Im}(t + 1) &= v_{\Im}(t) - h_{\Im}(t)z_{\Im}(t), \\    
%     z(t) &= \Theta(v_{\Im}(t) - T_{\Im}(t)),
% \end{align}
% for $t = 2, 4, \dots, 2K$ respectively
\begin{align}
    \hat{f}(z) = \sum_{t=0}^{K-1} (d_{\Re}(t) z_{\Re}(t) + \mathrm{j} \cdot d_{\Im}(t) z_{\Im}(t))  
\end{align} and $d_{\Re}, h_{\Re}, T_{\Re}, d_{\Im}, h_{\Im}, T_{\Im} \in \mathbb{R}^K$ computed by SGD as in \cite{stockl_optimized_2021}.
\item Training and Conversion Procedure for SpiNNaker2:
\begin{enumerate}
    \item Train S-LISTA and quantize to 4 bits, create populations/projections!
    \item Approximate $\mathcal{S}_{\alpha_t}(s) = \text{sign}(s)\text{ReLU}(s - \alpha_t)$ with Eq. \eqref{eq:fs_cmplx}!
    \item Generate spikes $z_{\Re}(t), z_{\Im}(t)$ by the FS approximation of identity!
\end{enumerate}
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.35\linewidth]{figures/s2_jetson.jpg}
    \caption*{Spinnaker2 board used in this work.}
    \label{fig:enter-label}
\end{figure}
% First, we perform quantization of the CNN weights, then create the neuron populations and projections by extracting the connection information between these populations. Afterwards, the soft-threshold operators in \eqref{eq:st} are approximated for each layer using the FS neuron model optimized for the specific threshold $\alpha_t$
% \textcolor{red}{TODO: \begin{enumerate}
%      \item High-level overview, DNN training (with or without FS activation), post training quantization,
%      Replacement of activations wih neurons, creating populations and connections from weights. 
%      At inference: spike encoding using FS identity (figure with nice workflow)
%      \item Complex valued FS neuron equations, difference from original paper, possible paralell impl.
%      \item Optimization: fixed function approximation, usage as activation
%      \item Optimization: Tips and tricks, diferentiable Heaviside approximation, etc.
%  \end{enumerate}}

==> sections/poster/preliminaries.tex <==
% \textcolor{red}{TODO: \begin{enumerate}
%      \item MHR formal definition, CS approach as constrained LS problem
%      \item FISTA and structured LISTA comparison (figure)
%      \item LISTA figure eventuell
%      \item Training loss, etc.
%  \end{enumerate}}
\begin{itemize}
    % \item Source parameters $\bm{\xi}_{p} = [\xi_{1p}, \xi_{2p}, \dots, \xi_{Mp}]^{\top} \in [-\frac{1}{2}, \frac{1}{2}]^{M}$ for $p=1,\dots, P$.
    % and $N_{1}, N_{2}, \dots N_{M}$ the number of sensors for each dimension. 
    % \item Measurement Model\cite{dimitri2010tensor}: \begin{align}\label{eq:sys_kr}
    % &\bm{y} = \bm{A}(\bm{\xi})\bm{b} + \bm{z} \in \mathbb{C}^{N} \\ 
    % &\bm{A}(\bm{\xi}) = \left(\bm{A}_{1}(\bm{\xi}) \ast \cdots \ast \bm{A}_{M}(\bm{\xi})\right) \\
    % &\bm{A}_{m}(\bm{\xi}) = [\bm{a}_{m}(\xi_{m1}), \dots, \bm{a}_{m}(\xi_{mP})] \in \mathbb{C}^{N_{m}\times P}\\
    % &\bm{a}_{m}(\xi_{mp}) \in \mathbb{C}^{N_{m}} \text{ with } \left(\bm{a}_{m}(\bm{\xi}_{mp})\right)_{k} = \mathrm{e}^{-\mathrm{j}2\pi \xi_{mp} k},
    % \end{align}
    % where $k = 0, \dots N_{m} - 1,\, N = \prod_{m=1}^{M} N_{m}$, $\bm{z}\sim\mathcal{N}(0, \frac{\sigma^{2}}{N} \bm{I})$ and $\ast$ Khatri-Rao product.
%      \item \textbf{Sparse Recovery:} Oversample dictionary $\bm{A}(\bm{\xi}) \in \mathbb{C}^{N\times L}$,
%  % \, L\gg P
%  solve
%  \begin{align}
%      \min_{\bm{b}\in\mathbb{C}^{L}} \left\lVert \bm{y} - \bm{A}(\bm{\xi})\bm{b} \right\rVert_{2}^{2} - \lambda\lVert \bm{b} \rVert_{1},
%  \end{align}
% and recover indices of non-zero elements!
\vspace{-1.5cm}
% \begin{align*}
%     &\bm{W}^{1}_{t}=\bm{A}^{H}(\bm{\xi}), \, \eta=\mu^{-1}_{\text{max}}(\bm{A}^{H}(\bm{\xi})\bm{A}(\bm{\xi})) \\
%     &\bm{W}^{2}_{t} = \bm{I} - {\eta}\bm{A}^{H}(\bm{\xi})\bm{A}(\bm{\xi})\\
%     &\bm{b}_t = \mathcal{S}_{\alpha/\eta}\left(\bm{W}^{1}_{t} \bm{y} + \bm{W}^{2}_{t} \bm{b}_{t-1}\right) \\
% &\mathcal{S}_{\alpha}(\bm{x}) = \text{sign}(\bm{u}) \max(\lvert\bm{u}\rvert - \alpha, \bm{0})
% \end{align*}
\begin{figure}
    \includegraphics[width=.6\linewidth]{figures/2024asilomar_fista.pdf}
    \caption*{Fast Iterative Shrinkage and Thresholding Algorithm}
    \label{fig:fista}
\end{figure}\vspace{-.5cm}
\item \textbf{S-LISTA\cite{fu2021structured}:} Unroll FISTA iterations and replace Toeplitz matrix multiplications by convolutions with learned kernels!
\begin{figure}
    \centering
    \includegraphics[width=.65\linewidth]{figures/2024asilomar_lista_small.pdf}
    \caption*{Structured Learned Iterative Shrinkage and Thresholding Algorithm}
    \label{fig:enter-label}
\end{figure}\vspace{-.5cm}
\item Training done on dataset $\mathcal{D} = \{(\bm{y}_{d}, \bm{b}_{d})\}_{d}^{D}$, with loss function
% \begin{align}
  $  \mathcal{L}(\bm{b}_d , \hat{\bm{b}}_d) = \frac{1}{D}\sum_{d=1}^{D} \lVert\bm{b}_d -  \hat{\bm{b}}_d \rVert_{2}^{2}/\lVert\bm{b}_d \rVert_2^{2}$
% \end{align}
\end{itemize}


==> sections/poster/preliminaries_col1.tex <==
\begin{itemize}
    \item Measurement Model\cite{dimitri2010tensor}: \begin{align}\label{eq:sys_kr}
    &\bm{y} = \bm{A}(\bm{\xi})\bm{b} + \bm{z} \in \mathbb{C}^{N} \\ 
    &\bm{A}(\bm{\xi}) = \left(\bm{A}_{1}(\bm{\xi}) \ast \cdots \ast \bm{A}_{M}(\bm{\xi})\right) \\
    &\bm{A}_{m}(\bm{\xi}) = [\bm{a}_{m}(\xi_{m1}), \dots, \bm{a}_{m}(\xi_{mP})] \in \mathbb{C}^{N_{m}\times P}\\
    &\bm{a}_{m}(\xi_{mp}) \in \mathbb{C}^{N_{m}} \text{ with } \left(\bm{a}_{m}(\bm{\xi}_{mp})\right)_{k} = \mathrm{e}^{-\mathrm{j}2\pi \xi_{mp} k},
    \end{align}
    \item \textbf{Goal:} Estimate $\bm{\xi} = \{\bm{\xi}_{p}\}_{p=1}^{P}$ given the measurement $\bm{y}$!
    \item \textbf{Sparse Recovery:} Oversample dictionary $\bm{A}(\bm{\xi}) \in \mathbb{C}^{N\times L}$,
 % \, L\gg P
 solve
 \begin{align}
     \min_{\bm{b}\in\mathbb{C}^{L}} \left\lVert \bm{y} - \bm{A}(\bm{\xi})\bm{b} \right\rVert_{2}^{2} - \lambda\lVert \bm{b} \rVert_{1},
 \end{align}
and recover indices of non-zero elements!
\item  \textbf{FISTA \cite{beck2009fista}:} Optimal recovery but many iterations needed!\vspace{1cm}
\end{itemize}
